Answer Set Programming Made Easy

We take up an idea from the folklore of Answer Set Programming, namely that choices, integrity constraints along with a restricted rule format is sufficient for Answer Set Programming. We elaborate upon the foundations of this idea in the context of the logic of Here-and-There and show how it can be derived from the logical principle of extension by definition. We then provide an austere form of logic programs that may serve as a normalform for logic programs similar to conjunctive normalform in classical logic. Finally, we take the key ideas and propose a modeling methodology for ASP beginners and illustrate how it can be used.

==> approach.tex <==
\section{Approach}\label{sec:approach}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> debugging.tex <==
\subsection{Debugging}
\label{sec:debugging}

Another application of optimization statements is debugging easy logic programs.
%
As mentioned, a special feature of austere logic programs (as well as the ones admitting stratified negation only)
is that inconsistencies are confined to the violation of integrity constraints
(rather than caused by odd loops spread over the program).
%
We can exploit this for debugging in the following way.
%
Replace each integrity constraint
\[
  \bot\leftarrow l_{m+1}\wedge\dots\wedge l_n
  \quad\text{ by }\quad
  \mathit{ic}(i)\leftarrow l_{m+1}\wedge\dots\wedge l_n
\]
where $\mathit{ic}$ is a new predicate symbol and $i$ an identifier for the integrity constraint at hand.
%
And add a minimization statement
\[
  \#\mathit{minimize}\{\mathit{ic}(I)\}
\]
to output only solution candidates with a minimum number of violations.
%
As an example, let us replace lines~8 to~10 in Listing~\ref{lp:ham} by
\begin{lstlisting}[firstnumber=8]
ic(unreached(V)) :- node(V), not reached(V).
  ic(two_out(V)) :- hc(V,U), hc(V,W), U!=W.
   ic(two_in(V)) :- hc(U,V), hc(W,V), U!=W.

#minimize{ ic(I) }.
\end{lstlisting}
The purpose of the optimization directive in Line~12 is to restrict the stable models to the ones violating the fewest constraints in lines~8-10.
Hence, if there are proper solutions satisfying all integrity constraints, they are output and no others.

Note that the above introduction of new consequents yields normal yet stratified rules.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> include/asp-macros/dtel.tex <==
\RequirePackage{bm}
\RequirePackage{textcomp}
\RequirePackage{upgreek}

\IfFileExists{outline.tex}{\input{outline}}{}

\newcommand{\tuple}[1]{\langle #1 \rangle}
\renewcommand{\H}{\ensuremath{\mathbf{H}}} % REDEFINITION
\newcommand{\T}{\ensuremath{\mathbf{T}}}
\newcommand{\M}{\ensuremath{\mathbf{M}}}

\newcommand{\next}{\text{\rm \raisebox{-.5pt}{\Large\textopenbullet}}}  % {{\ensuremath{\circ}}}
\newcommand{\previous}{\text{\rm \raisebox{-.5pt}{\Large\textbullet}}}  % {{\ensuremath{\bullet}}}
\newcommand{\wnext}{\ensuremath{\widehat{\next}}}
\newcommand{\wprevious}{\ensuremath{\widehat{\previous}}}
\newcommand{\alwaysF}{\ensuremath{\square}}
\newcommand{\alwaysP}{\ensuremath{\blacksquare}}
\newcommand{\eventuallyF}{\ensuremath{\Diamond}}
\newcommand{\eventuallyP}{\ensuremath{\blacklozenge}}
\IfFileExists{outline.tex}
        {\newcommand{\until}{\ensuremath{\mathbin{\mbox{\outline{$\bm{\mathsf{U}}$}}}}}}
        {\newcommand{\until}{\ensuremath{\mathbin{\bm{\mathsf{U}}}}}}
\IfFileExists{outline.tex}
        {\newcommand{\release}{\ensuremath{\mathbin{\mbox{\outline{$\bm{\mathsf{R}}$}}}}}}
        {\newcommand{\release}{\ensuremath{\mathbin{\bm{\mathsf{R}}}}}}
\newcommand{\since}{\ensuremath{\mathbin{\bm{\mathsf{S}}}}}
\newcommand{\trigger}{\ensuremath{\mathbin{\bm{\mathsf{T}}}}}
\IfFileExists{outline.tex}
        {\newcommand{\finally}{\ensuremath{\mbox{\outline{$\bm{\mathsf{F}}$}}}}}
        {\newcommand{\finally}{\ensuremath{\bm{\mathsf{F}}}}}
\newcommand{\initially}{\ensuremath{\bm{\mathsf{I}}}}

\newcommand{\stp}{\ensuremath{\uptau}}

\newcommand{\dalways}[1]{\ensuremath{[#1]\,}}                        % \DBox
\newcommand{\deventually}[1]{\ensuremath{\langle#1\rangle\,}}        % \DDia
\newcommand{\drel}[2]{\ensuremath{{\parallel}{#1}{\parallel}^{#2}}}  % \Rel

\newcommand{\intervc}[2]{[#1..#2]}
\newcommand{\intervo}[2]{[#1..#2)}
\newcommand{\ointerv}[2]{(#1..#2]}
\newcommand{\rangec}[3]{#1 \in \intervc{#2}{#3}}
\newcommand{\rangeo}[3]{#1 \in \intervo{#2}{#3}}
\newcommand{\orange}[3]{#1 \in \ointerv{#2}{#3}}


==> include/asp-macros/listings.tex <==
% The language definitions below require the following packages:
%
%     \usepackage{courier}
%     \usepackage{xcolor}
%     \usepackage{relsize}
%
%     \input{listings}
%     \renewcommand{\Underscore}{\textscale{1}{\textunderscore}}
%
% Without extra packages I had to provide an alternative underscore definition
% to get decent looking underscores.
%
% As an alternative to courier, it is also possible to use the `lmodern`
% package.
%
%     \usepackage[T1]{fontenc}
%     \usepackage{lmodern}
%     \usepackage{xcolor}
%     \usepackage{relsize}
%
%     \input{listings}
%
% When the python or clingo language is given, tex code can be embedded
% escaping it in `#( ... #)`, which is treated like a comment in Python.
% Furthermore, for logic programs the character sequence is `%%` is not output.
% This can be used to add labels at the end of lines. For example, in a logic
% program one can write
%
%     H :- B.%%#( \label{lst:rule} #)
%
% to refer to the rule from the document without having to worry about changing
% line numbers when refactoring. The annotated program will still be runnable
% with clingo.

\providecommand{\Underscore}{\textunderscore}

\lstdefinelanguage{clingo}{%
  basicstyle=\ttfamily,%
  keywordstyle=[1]\bfseries,%
  keywordstyle=[2]\bfseries,%
  keywordstyle=[3]\bfseries,%
  showstringspaces=false,%
  literate={_}{\Underscore}1 {\%\%}{}0,%
  escapeinside={\#(}{\#)},%
  alsoletter={\#,\&},%
  keywords=[1]{not,from,import,def,if,else,elif,return,while,break,and,or,for,in,del,and,class,with,as,is,yield,async},%
  keywords=[2]{\#const,\#show,\#minimize,\#base,\#theory,\#count,\#external,\#program,\#script,\#end,\#heuristic,\#edge,\#project,\#show,\#sum},%
  keywords=[3]{&,&dom,&sum,&diff,&show},%
  morecomment=[l]{\#\ },%
  morecomment=[l]{\%\ },%
  morestring=[b]",%
  stringstyle={\itshape},%
  commentstyle={\color{darkgray}}%
}

\lstdefinelanguage{python}{%
  basicstyle=\ttfamily,%
  keywordstyle=[1]\bfseries,%
  showstringspaces=false,%
  literate={_}{\Underscore}{1},%
  escapeinside={\#(}{\#)},%
  alsoletter={\#,\&},%
  keywords=[1]{not,from,import,def,if,else,elif,return,while,break,and,or,for,in,del,and,class,with,as,is,yield,async},%
  morecomment=[l]{\#\ },%
  morestring=[b]",%
  stringstyle={\itshape},%
  commentstyle={\color{darkgray}}%
}



==> include/asp-macros/logics.tex <==
\newcommand{\HT}{\ensuremath{\mathrm{HT}}}
\newcommand{\EL}{\ensuremath{\mathrm{EL}}}
%
\newcommand{\LTL}{\ensuremath{\mathrm{LTL}}}
\newcommand{\LTLf}{\ensuremath{\mathrm{LTL}_{\!f}}}
\newcommand{\LTLo}{\ensuremath{\mathrm{LTL}_{\omega}}}
\newcommand{\THT}{\ensuremath{\mathrm{THT}}}
\newcommand{\THTf}{\ensuremath{\mathrm{THT}_{\!f}}}
\newcommand{\THTo}{\ensuremath{\mathrm{THT}_{\!\omega}}}
\newcommand{\TEL}{\ensuremath{\mathrm{TEL}}}
\newcommand{\TELf}{\ensuremath{{\TEL}_{\!f}}}
\newcommand{\TELo}{\ensuremath{{\TEL}_{\omega}}}
%
\newcommand{\LDL}{\ensuremath{\mathrm{LDL}}}
\newcommand{\LDLf}{\ensuremath{\mathrm{LDL}_{\!f}}}
\newcommand{\LDLo}{\ensuremath{\mathrm{LDL}_{\omega}}}
\newcommand{\DHT}{\ensuremath{\mathrm{DHT}}}
\newcommand{\DHTf}{\ensuremath{\mathrm{DHT}_{\!f}}}
\newcommand{\DHTo}{\ensuremath{\mathrm{DHT}_{\!\omega}}}
\newcommand{\DEL}{\ensuremath{\mathrm{DEL}}}
\newcommand{\DELf}{\ensuremath{{\DEL}_{\!f}}}
\newcommand{\DELo}{\ensuremath{{\DEL}_{\omega}}}
%
\newcommand{\DL}{\ensuremath{\mathrm{DL}}}


==> include/asp-macros/nogoods.tex <==
\newcommand{\domain}[1]{\ensuremath{\mathit{dom}(#1)}}

\newcommand{\ass}{\ensuremath{A}}

\newcommand{\tlits}[1]{\ensuremath{{#1}^{\true}}}
\newcommand{\flits}[1]{\ensuremath{{#1}^{\false}}}
\newcommand{\prefix}[2]{\ensuremath{#1[#2]}}

% \newcommand{\clno}[1]{\ensuremath{\delta(#1)}}
% \newcommand{\ClNo}[1]{\ensuremath{\Delta(#1)}}
% \newcommand{\nocl}[1]{\ensuremath{\gamma(#1)}}
% \newcommand{\NoCl}[1]{\ensuremath{\Gamma(#1)}}

\newcommand{\CN}[1]{\ensuremath{\Delta_{#1}}}
\newcommand{\LN}[1]{\ensuremath{\Lambda_{#1}}}

\newcommand{\dl}[0]{\ensuremath{\mathit{dl}}}
\newcommand{\dlevel}[1]{\ensuremath{\mathit{dlevel}(#1)}}
\newcommand{\opp}[1]{\ensuremath{\overline{#1}}}

\newcommand{\undef}[0]{\ensuremath{\circ}}
\newcommand{\trdef}[0]{\ensuremath{\times}}
\newcommand{\scc}[1]{\ensuremath{\mathit{scc}(#1)}}
\newcommand{\source}[1]{\ensuremath{\mathit{source}(#1)}}


==> include/asp-macros/operators.tex <==

% - operators ------------------------------------------------------------------
\newcommand{\Cn}[1]{\ensuremath{\mathit{Cn}(#1)}}
\newcommand{\reduct}[2]{\ensuremath{#1^{#2}}}

\newcommand{\Top}[1]{\ensuremath{T_{#1}}}
\newcommand{\T}[2]{\Top{#1}#2}
\newcommand{\Topi}[2]{\Top{#2}^{#1}}
\newcommand{\Ti}[3]{\Topi{#1}{#2}#3}

\newcommand{\BF}[1]{\ensuremath{\mathit{BF}(#1)}}
\newcommand{\CF}[1]{\ensuremath{\mathit{CF}(#1)}}
\newcommand{\CFIF}[1]{\ensuremath{\overleftarrow{\mathit{CF}}(#1)}}
\newcommand{\CFFI}[1]{\ensuremath{\overrightarrow{\mathit{CF}}(#1)}}
\newcommand{\CFX}[1]{\ensuremath{\mathit{CF}^x(#1)}}

\newcommand{\loops}[1]{\ensuremath{\mathit{loop}(#1)}}\message{*** loop already defined ***}
\newcommand{\ES}[2]{\ensuremath{\mathit{ES}_{\!#2}(#1)}}
\newcommand{\EB}[2]{\ensuremath{\mathit{EB}_{\!#2}(#1)}}
\newcommand{\LFM}[2]{\ensuremath{\mathit{LF}_{\!#2}(#1)}}
\newcommand{\LF}[1]{\ensuremath{\mathit{LF}(#1)}}

% - semantic operators -----------------------------------------------------------
\newcommand{\SM}[1]{\ensuremath{\mathit{SM}(#1)}}


==> include/asp-macros/outline.tex <==
\RequirePackage{xcolor}
\makeatletter

%%% MALIPIVO's PDF SPECIAL TO CHANGE FONT OUTLINE THICKNESS/COLOR
% https://tex.stackexchange.com/questions/18472/tikz-halo-around-text/169549#169549
\input pdf-trans
\newbox\qbox
\def\usecolor#1{\csname\string\color@#1\endcsname\space}
\newcommand\bordercolor[1]{\colsplit{1}{#1}}
\newcommand\fillcolor[1]{\colsplit{0}{#1}}
\newcommand\outline[1]{\leavevmode%
  \def\maltext{#1}%
  \setbox\qbox=\hbox{\maltext}%
  \boxgs{Q q 2 Tr \thickness\space w \fillcol\space \bordercol\space}{}%
  \copy\qbox%
}
\makeatother
\newcommand\colsplit[2]{\colorlet{tmpcolor}{#2}\edef\tmp{\usecolor{tmpcolor}}%
  \def\tmpB{}\expandafter\colsplithelp\tmp\relax%
  \ifnum0=#1\relax\edef\fillcol{\tmpB}\else\edef\bordercol{\tmpC}\fi}
\def\colsplithelp#1#2 #3\relax{%
  \edef\tmpB{\tmpB#1#2 }%
  \ifnum `#1>`9\relax\def\tmpC{#3}\else\colsplithelp#3\relax\fi
}
\bordercolor{black}
\fillcolor{white}
\def\thickness{.3}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> include/asp-macros/syntax.tex <==
\newcommand{\naf}[1]{\ensuremath{{\sim\!{#1}}}}

\newcommand{\head}[1]{\ensuremath{\mathit{head}(#1)}}
\newcommand{\body}[1]{\ensuremath{\mathit{body}(#1)}}

\newcommand{\atom}[1]{\ensuremath{\mathit{atom}(#1)}}

\newcommand{\poslits}[1]{\ensuremath{{#1}^+}}
\newcommand{\neglits}[1]{\ensuremath{{#1}^-}}

\newcommand{\pbody}[1]{\poslits{\body{#1}}}
\newcommand{\nbody}[1]{\neglits{\body{#1}}}

\newcommand{\PRG}{\ensuremath{P}}

\newcommand{\atbody}[2]{\ensuremath{\mathit{body}_{#1}(#2)}}

\newcommand{\ground}[1]{\ensuremath{\mathit{grd}(#1)}}


==> include/asp-macros/systems.tex <==
\newcommand{\sysfont}{\textit}
\newcommand{\acthex}{\sysfont{acthex}}
\newcommand{\adsolver}{\sysfont{adsolver}}
\newcommand{\anthem}{\sysfont{anthem}}
\newcommand{\asparagus}{\sysfont{asparagus}}
\newcommand{\aspartame}{\sysfont{aspartame}}
\newcommand{\aspic}{\sysfont{aspic}}
\newcommand{\aspcud}{\sysfont{aspcud}}
\newcommand{\aspmt}{\sysfont{aspmt}}
\newcommand{\asprilo}{\sysfont{asprilo}}
\newcommand{\asprin}{\sysfont{asprin}}
\newcommand{\assat}{\sysfont{assat}}
\newcommand{\autofolio}{\sysfont{autofolio}}
\newcommand{\berkmin}{\sysfont{berkmin}}
\newcommand{\caspo}{\sysfont{caspo}}
\newcommand{\chuffed}{\sysfont{chuffed}}
\newcommand{\chasp}{\sysfont{chasp}}
\newcommand{\claspD}{\sysfont{claspD}}
\newcommand{\claspar}{\sysfont{claspar}}
\newcommand{\claspfolio}{\sysfont{claspfolio}}
\newcommand{\clasp}{\sysfont{clasp}}
\newcommand{\claspre}{\sysfont{claspre}}
\newcommand{\clingcon}{\sysfont{clingcon}}
\newcommand{\clingo}{\sysfont{clingo}}
\newcommand{\cmodels}{\sysfont{cmodels}}
\newcommand{\coala}{\sysfont{coala}}
\newcommand{\cplex}{\sysfont{cplex}}
\newcommand{\dingo}{\sysfont{dingo}}
\newcommand{\dflat}{\sysfont{dflat}}
\newcommand{\dlvhex}{\sysfont{dlvhex}}
\newcommand{\dlv}{\sysfont{dlv}}
\newcommand{\ezcsp}{\sysfont{ezcsp}}
\newcommand{\ezsmt}{\sysfont{ezsmt}}
\newcommand{\embasp}{\sysfont{embasp}}
\newcommand{\fastdownward}{\sysfont{fastdownward}}
\newcommand{\ftolp}{\sysfont{f2lp}}
\newcommand{\gasp}{\sysfont{gasp}}
\newcommand{\gfd}{\sysfont{g12fd}}
\newcommand{\gecode}{\sysfont{gecode}}
\newcommand{\gidl}{\sysfont{gidl}}
\newcommand{\ginkgo}{\sysfont{ginkgo}}
\newcommand{\gnt}{\sysfont{gnt}}
\newcommand{\gringo}{\sysfont{gringo}}
\newcommand{\harvey}{\sysfont{harvey}}
\newcommand{\iclingo}{\sysfont{iclingo}}
\newcommand{\idp}{\sysfont{idp}}
\newcommand{\inca}{\sysfont{inca}}
\newcommand{\jdlv}{\sysfont{jdlv}}
\newcommand{\lctocasp}{\sysfont{lc2casp}}
\newcommand{\lparse}{\sysfont{lparse}}
\newcommand{\lpsolve}{\sysfont{lpsolve}}
\newcommand{\lptodiff}{\sysfont{lp2diff}}
\newcommand{\lptosat}{\sysfont{lp2sat}}
\newcommand{\mchaff}{\sysfont{mchaff}}
\newcommand{\measp}{\sysfont{measp}}
\newcommand{\metasp}{\sysfont{metasp}}
\newcommand{\mingo}{\sysfont{mingo}}
\newcommand{\minisat}{\sysfont{minisat}}
\newcommand{\minisatid}{\sysfont{minisatid}}
\newcommand{\minizinc}{\sysfont{minizinc}}
\newcommand{\mznfzn}{\sysfont{mzn2fzn}}
\newcommand{\nomorepp}{\sysfont{nomore++}}
\newcommand{\oclingo}{\sysfont{oclingo}}
\newcommand{\omiga}{\sysfont{omiga}}
\newcommand{\piclasp}{\sysfont{piclasp}}
\newcommand{\picosat}{\sysfont{picosat}}
\newcommand{\picat}{\sysfont{picat}}
\newcommand{\picatsat}{\sysfont{picatsat}}
\newcommand{\plasp}{\sysfont{plasp}}
\newcommand{\quontroller}{\sysfont{quontroller}}
\newcommand{\reify}{\sysfont{reify}}
\newcommand{\rosoclingo}{\sysfont{rosoclingo}}
\newcommand{\sag}{\sysfont{sag}}
\newcommand{\satz}{\sysfont{satz}}
\newcommand{\siege}{\sysfont{siege}}
\newcommand{\smac}{\sysfont{smac}}
\newcommand{\smodelscc}{\sysfont{smodels$_{\!cc}$}}
\newcommand{\smodelsr}{\sysfont{smodels}$_r$}
\newcommand{\smodels}{\sysfont{smodels}}
\newcommand{\stelp}{\sysfont{stelp}}
\newcommand{\sugar}{\sysfont{sugar}}
\newcommand{\teaspoon}{\sysfont{teaspoon}}
\newcommand{\tel}{\sysfont{tel}}
\newcommand{\telingo}{\sysfont{telingo}}
\newcommand{\unclasp}{\sysfont{unclasp}}
\newcommand{\wasp}{\sysfont{wasp}}
\newcommand{\xorro}{\sysfont{xorro}}
\newcommand{\zchaff}{\sysfont{zchaff}}
\newcommand{\zzz}{\sysfont{z3}}

\newcommand{\clingoM}[1]{\clingo{\small\textnormal{[}\textsc{#1}\textnormal{]}}}
\newcommand{\ASPm}[1]{ASP\raisebox{.7pt}{[\textsc{#1}]}}

\newcommand{\flatzinc}{\sysfont{FlatZinc}}
\newcommand{\aspif}{\sysfont{aspif}}

\newcommand{\python}{Python}
\newcommand{\lua}{Lua}
\newcommand{\cpp}{C++}
\newcommand{\C}{C}
\newcommand{\java}{Java}
\newcommand{\haskell}{Haskell}


==> include/asp-macros/tableau.tex <==
\newcommand{\true}{\ensuremath{\boldsymbol{T}}}
\newcommand{\false}{\ensuremath{\boldsymbol{F}}}

\newcommand{\Tsigned}[1]{\ensuremath{\true{#1}}}\message{ *** RENAME, Tlit,Flit ?? *** }
\newcommand{\Fsigned}[1]{\ensuremath{\false{#1}}}

\newcommand{\TOP}[1]{\ensuremath{D_{#1}}}
\newcommand{\COP}[1]{\ensuremath{D^*_{#1}}}

\newcommand{\Proviso}[1]{\raisebox{-7pt}[0pt][0pt]{\ensuremath{(#1)}}}

\newcommand{\plit}[1]{\ensuremath{\boldsymbol{t}{#1}}}
\newcommand{\nlit}[1]{\ensuremath{\boldsymbol{f}{#1}}}


==> inconsistency.tex <==
\section{Inconsistency in Austere Logic Programs}

\begin{itemize}
	\item 
		In normal logic, inconsistency is caused by odd loops.
	\item 
		An inconsistent logic program:
		\begin{align*}
			a\leftarrow& \\
			e\leftarrow& \\
			b\leftarrow& c \wedge e \\
			c\leftarrow& a\wedge \neg d \\
			d\leftarrow& b
		\end{align*}
		Here the inconsistency is caused by the odd loop formed due to the last three rules.
	\item 
		But not odd loops cause inconsistency. 
		%
		Some odd loops are used to remove unwanted answer sets like the integrity constraint in the last rule of the program below.
		\begin{align*}
			a\leftarrow& \neg b \\
			b\leftarrow& \neg a \\
			c\leftarrow& b \wedge d \\
			d\leftarrow& a \wedge \neg c 
		\end{align*}
		Integrity constraints are used for this purpose.
	\item 
		We see that the odd loops are important but for ensuring consistency, we can not limit the checking process to a specific segment of the program like in case of austere programs. 
	\item
		Instead austere programs can be used to express odd loops and in this case we can limit our consistency checking to the integrity constraints in the program.
\end{itemize}

==> optimization.tex <==
\subsection{Optimization}
\label{sec:optimization}

Strictly speaking, optimization statements do not belong to a logic program and are rather instructions to an ASP system.
%
Since they take predicates as argument but refrain from deriving any predicates,
it is natural to state them at the end of a program.

For instance, we can turn the formalization of the Hamiltonian circuit problem in Listing~\ref{lp:ham} into one of the Traveling salesperson problem
by adding edge costs to the facts in lines 1-3, such as
\begin{lstlisting}[firstnumber=2]
cost(1,2,3). cost(2,3,5). cost(2,4,6). cost(3,1,4).
cost(3,4,7). cost(4,1,5). cost(4,3,7).
\end{lstlisting}
along with an optimization directive of the form:
\begin{lstlisting}[firstnumber=12]
#minimize { C,X,Y : hc(X,Y), cost(X,Y,C) }.
\end{lstlisting}
This statement tells the solver to search for solutions having a cost minimal Hamiltonian circuit;
it naturally extends the stratification of the easy program, since it only refers to predicates defined in previous lines,
and does not contribute to the formation but only the selection of stable models, just like integrity constraints.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

